Intrinsic Physical Concepts Discovery with Object-Centric Predictive Models

The ability to discover abstract physical concepts and understand how they work in the world through observing lies at the core of human intelligence. The acquisition of this ability is based on compositionally perceiving the environment in terms of objects and relations in an unsupervised manner. Recent approaches learn object-centric representations and capture visually observable concepts of objects, e.g., shape, size, and location. In this paper, we take a step forward and try to discover and represent intrinsic physical concepts such as mass and charge. We introduce the PHYsical Concepts Inference NEtwork (PHYCINE), a system that infers physical concepts in different abstract levels without supervision. The key insights underlining PHYCINE are two-fold, commonsense knowledge emerges with prediction, and physical concepts of different abstract levels should be reasoned in a bottom-up fashion. Empirical evaluation demonstrates that variables inferred by our system work in accordance with the properties of the corresponding physical concepts. We also show that object representations containing the discovered physical concepts variables could help achieve better performance in causal reasoning tasks, i.e., ComPhy.

==> f4.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width = 0.45\textwidth]{f_4.pdf}
    \vspace{-5pt}
    \caption{Illustration of how PHYCINE imagines the unseen future. $N$ time steps are given to estimate the object representations of the first time step. In addition to being capable of re-generating $x^{0:N}$, $z^0$ can also predict $x^{N:T}$.  }
    \label{fig:task-pred}
    \vspace{-10pt}
\end{figure}

==> t1.tex <==
\begin{table*}[t!]
	\centering
	\caption{Performance (per question/option accuracy) comparison with the state-of-the-art methods MAC (V+), NS-DR, DCL, and ALOE on CLEVRER, ALOE takes static scene representations from Monet as visual input while ODDN-ALOE use representations of ODDN.}
	%\resizebox{\textwidth}{!}{
	\begin{tabular}{cccccccc}
	\hline
		Model & Descriptive & \multicolumn{2}{c}{Explanatory} & \multicolumn{2}{c}{Predictive}& \multicolumn{2}{c}{Counterfactual} \\
		&  & per opt. & per ques. & per opt. & per ques. &per opt. &per ques. \\ \hline
		MAC(V+) & 86.4 &  70.5 & 22.3 & 59.7 &42.9 &63.5 &25.1 \\ 
	    NS-DR & 88.1 &  87.6 & 79.6 & 82.9 & 68.7 &74.1 &42.2 \\\
	    DCL & 90.7 &  89.6 & 82.8 & 90.5 & 82.0 &80.4 &46.5 \\
	    ALOE&94.0 & 98.5 & 96.0 &93.5 &87.5 &91.4 &75.6 \\\hline
	    ODDN-ALOE & \textbf{95.8} & \textbf{98.9} & \textbf{97.0} & \textbf{95.7} &\textbf{91.8} &\textbf{93.0} &\textbf{80.1} \\\hline
	\end{tabular}%
	%}
	\label{tab:dim}%
	\vspace{-10pt}
\end{table*}%

